Non-thermal motions and atmospheric heating of cool stars

The magnetic processes associated with the non-thermal broadening of optically thin emission lines appear to carry enough energy to heat the corona and accelerate the solar wind. We investigate whether non-thermal motions in cool stars exhibit the same behaviour as on the Sun by analysing archival stellar spectra taken by the Hubble Space Telescope, and full-disc Solar spectra taken by the Interface Region Imaging Spectrograph. We determined the non-thermal velocities by measuring the excess broadening in optically thin emission lines formed in the stellar atmosphere; the chromosphere, the transition region and the corona. Assuming the non-thermal broadening is caused by the presence of Alfv\'en waves, we also determined the associated wave energy densities. Our results show that, with a non-thermal velocity of $\sim$23 kms$^{-1}$ the Sun-as-a-star results are in very good agreement with values obtained from spatially-resolved solar observations. The non-thermal broadening in our sample show correlation to stellar rotation, with the strength of the non-thermal velocity decreasing with decreasing rotation rate. Finally, the non-thermal velocity in cool Sun-like stars varies with atmospheric height or temperature of the emission lines, and peaks at transition region temperatures. This points towards a solar-like Alfv\'en wave driven heating in stellar atmospheres. However, the peak is at a lower temperature in some cool stars suggesting that, other magnetic process such as flaring events could also dominate.

==> final_table.tex <==
\startlongtable
\begin{deluxetable*}{lcccccccccc}
\tabletypesize{\footnotesize}
\tablewidth{0.99\textwidth}
\tablecaption{ \label{table1} Stellar properties \label{table1}}
\tablehead{
\colhead{HD name}             &other name  &\colhead{mass}              &\colhead{radius}              &\colhead{$T_\mathrm{eff}$}              &\colhead{$v_\mathrm{rad}$}
              &\colhead{$P_\mathrm{rot}$}               &\colhead{$\log {R'_\mathrm{HK}}$}              &\colhead{$\xi_\mathrm{Si1393}$}              &\colhead{planet host}              &\colhead{additional refs}
\\
&&$\mathrm{M_\odot}$ &$\mathrm{R_\odot}$&K&km~s$^{-1}$&days& &km~s$^{-1}$& &
}
\startdata
HD 75732              &55 Cnc       &0.92    &0.95    &5235      &27.8     &42.0             &-5.01      &    25.9   &Yes               &1, 2\\                                  
HD 129333             &EK Dra       & 0.89   &0.91    &5845      &-20.0    &2.6              &-4.10      &    38.0   &No               &1, 3\\                                 
HD 209458             &	HIP 108859  &1.10    &1.1     &6099      &-14.7    &11.4             &-4.88      &    25.4   &Yes               &4, 5\\                                  
HD 69830              &LHS 245      & 0.86   &0.90    &5361      &32.2     &41.2             &-5.02      &    24.9   &Yes               &1\\                                     
HD 154345             &LHS 3260     &0.90    &0.84    &5468      &-46.6    &31.0             &-4.80      &    23.9   &Yes                &1\\                                    
HD 204961             & GJ 832      &0.45    &0.48    &3472      &13.0     &40.0             &-5.07      &    14.8   &Yes               &1, 6\\                                  
HD 38529              &	HIP 27253   &..      &..      &5697      &30.0     &35.7             &..           &    35.2   &Yes                 &1\\                                   
..                    &LTT 2050     &0.48    &0.45    &3633      &-6.7     &3.7              &..           &    14.7   &No                 &7, 8\\                               
..                    &LP 415-1619  &..      &0.58    &3420      &55.0     &..               &..           &    26.3   &No                 &1, 9, 10\\                           
HD 121504             &LTT 5432     &1.18&..      &6075      &19.6     &8.6              &-4.75      &    29.7   &Yes               &1, 11\\                                 
..                    &GJ 3470      &0.45&0.42    &3600      &26.3     &20.7             &..           &    17.8   &Yes                 &12, 13\\                              
HD 3651               &54 Psc       & 0.80 &0.88    &5221      &-32.9    &37.0             &-5.11      &    22.4   &Yes               &1\\                                     
HD 38459              &LTT 2361     &0.88&..      &5320      &26.0     &12.0             &-4.46      &    17.1   &No               &14, 15\\                               
HD 97658              &GJ 3651      & 0.90&0.74    &5148      &-1.5     &38.5             &-5.04      &    20.4   &Yes               &1\\                                     
..                    &WASP-69      &0.83    &0.81    &4715      &-9.4     &23.1             &..           &    21.1   &Yes                 & 1,16\\                               
HD 172669             &	HIP 91210   &1.08    &1.00    &5964      &-6.7     &..               &..           &    17.2   &No                 &17, 18\\                             
HD 1461               &LTT 149      &1.14    &1.10    &5765      &-10.0    &29.0             &-5.33      &    28.9   &Yes               &1\\                                     
HD 95128              &47 UMa       &1.29    &1.22    &5882      &11.5     &24.0             &-4.90      &    29.3   &Yes                &1\\                                    
HD 285968             &GJ 176       &0.45    &0.45    &3416      &26.0     &38.9             &-4.76      &    15.9   &Yes               &1,19, 20\\                              
HD 62850              &	HIP 37563   &1.01    &1.05    &5700      &17.9     &..               &-4.27      &    31.4   &No               &21, 22, 23, 24\\         
HD 22049              &$\epsilon$ Eri  &0.71    &0.72    &5146      &16.0     &11.7             &-4.50      &    23.2   &Yes                &1\\                                    
HD 13445              &GJ 86    &0.93    &0.80    &5151      &55.0     &30.0             &..           &    19.4   &Yes                 &1\\                                   
HD 7924               &HIP 6379 &0.80    &0.75    &5177      &-22.0    &38.0             &-4.90      &    18.2   &Yes                &1\\                                    
..                    &HAT-P-11    &0.81    &0.75    &4780      &-63.7    &30.5             &-4.65      &    18.7   &Yes               &1, 25\\                                 
HD 189733             &GJ 4130&0.82    &0.76    &5050      &-2.3     &13.4             &-4.50      &    21.8   &Yes                &1, 26\\                                
HD 156384C            &GJ 667 C&0.33    &..      &3600      &6.0      &105.0            &-5.30      &    10.4   &Yes                &1, 27, 28, 29 \\                       
HD 40307              &	GJ 2046&0.78    &0.71    &4827      &31.3     &48.0             &-5.25      &    20.1   &Yes               &1\\                                     
..                    &GJ 849  &0.49    &0.46    &3601      &-32.0    &39.2             &-4.95      &    15.7   &Yes               & 30, 31, 32 \\                          
HD 146233             &18 Sco& 0.98   &1.02    &5791      &10.0     &..               &-4.90      &    24.8   &No                &\\                                    
HD 104067             &LTT 4461& 0.91   &0.75    &4956      &15.0     &34.7             &-4.80      &    18.4   &Yes                &1\\                                    
HD 128311             &	GJ 3860& 1.32   &0.73    &4965      &-9.0     &14.0             &-4.49      &    23.6   &Yes               &1\\                                     
HD 136118             &	HIP 74948& 1.25   &1.74    &6097      &-3.0     &12.2             &-4.79      &    23.8   &No               &1\\                                    
HD 201091             &61 Cyg A&0.66    &0.67    &4545      &-65.5    &35.0             &-4.70      &    19.8   &No                & 33, 34 \\                            
HD 41004              &	HIP 28393&0.70    &..      &5010      &42.5     &27.0             &-4.67      &    23.6   &Yes               &35\\                                    
HD 99492              &83 Leo B& 1.24   &0.76    &4955      &3.0      &45.0             &-5.00      &    17.7   &Yes                &1\\                                    
HD 10647              &q1 Eri& 0.98   &1.10    &6105      &27.6     &10.0             &..           &    26.0   &Yes                 &1\\                                   
..                    &GJ 876  &0.37    &0.38    &3130      &-1.5     &81.0             &-5.00      &    13.6   &Yes                & 36, 37\\                              
HD 92788              &LTT 3928& 1.64   &0.99    &5836      &-4.0     &31.7             &-4.95      &    17.9   &Yes               &1\\                                     
HD 150706             &GJ 632&1.17    &0.96    &5961      &-17.0    &..               &-4.40      &    25.1   &Yes                &38\\                                   
HD 39091              &$\pi$ Men&1.12    &1.15    &5950      &10.0     &33.9             &-4.89      &    30.3   &Yes               &1\\                                     
HD 85512              &LHS 2201&0.69    &..      &4715      &-10.0    &47.1             &-4.96      &    17.0   &Yes               &1, 39\\                                 
HD 192263             &	HIP 99711& 0.83   &0.75    &4975      &-10.0    &24.5             &-4.57      &    18.0   &Yes               &1\\                                     
..                    &GJ 581 &0.31    &0.29    &3498      &-16.0    &94.2             &-5.43      &    9.9   &Yes               &1, 40, 41\\                             
HD 143761             &$\rho$ CrB            & 1.47   &1.32    &5823      &18.0     &18.5             &-4.95      &    18.0   &Yes               &1\\                                     
HD 186427             &16 Cyg B& 1.10   &1.15    &5674      &-28.0    &29.1             &-4.90      &    27.1   &Yes                &1\\                                    
HD 72905              &$\pi^1$ UMa&1.00    &0.96    &5873      &-12.0    &5.0              &-4.30      &    27.0   &No                & 42, 43, 44\\                         
HD 161897             &	HIP 86540& 1.01   &0.86    &5623      &-16.5    &..               &-4.77      &    17.7   &No               &\\                                     
HD 192310             &LHS 488& 0.84   &0.81    &5080      &-54.0    &47.7             &-5.30      &    16.8   &Yes                &1\\                                    
HD 24636              &HIP 17764&1.39    &1.37    &6831      &14.5     &..               &..           &    57.6   &No                 &17, 23, 45 \\                        
HD 25825              &LP 15-582& 1.01   &1.08    &5941      &37.0     &..               &-4.34      &    23.3   &No               &\\                                     
HD 160691             &$\mu$ Ara&1.08    &..      &5813      &-12.0    &31.0             &-4.97      &    22.0   &Yes              &46,47\\                     
HD 39587              &$\chi^1$ Ori& 0.82   &1.01    &5882      &-13.4    &5.2              &-4.40      &    30.7   &No               &\\                   
HD 186408             &16 Cyg A& 1.25   &1.25    &5781      &-27.5    &26.9             &-4.98      &    25.5   &No                &1\\                  
HD 197037             &LTT 16037 &1.11    &1.15    &6150      &8.0      &19.1                       &..&    18.8   &Yes               &1,48\\                    
HD 1835               &9 Cet& 0.98   &0.96    &5837      &-2.5     &..               &-4.40      &    29   &No                &\\     
\enddata
\tablecomments{Columns 1 to 9: HD name, other name, mass, radius, effective temperature, radial velocity, rotation, stellar activity 
or $\log {R'_\mathrm{HK}}$, mean non-thermal velocity determined in this work from the \ion{Si}{4} 1393 \AA~line. 
The stellar parameters are taken from \citet{valenti05} or the following references,
\citet{france18}$^1$; \citet{poppenhaeger10}$^2$; \citet{wright11}$^3$;\citet{silvavalio08}$^4$;
\citet{borosaikia18}$^5$; \citet{wittenmyer14}$^6$; \citet{schweitzer19}$^7$; \citet{passegger20}$^8$;
\citet{kopytova16}$^9$; \citet{terrien15}$^{10}$; \citet{mayor04}$^{11}$; \citet{bonfils12}$^{12}$;
\citet{palle20}$^{13}$; \citet{pavlenko19}$^{14}$; \citet{hojjatpanah20}$^{15}$; \citet{anderson14}$^{16}$;
\citet{mcdonald12}$^{17}$; \citet{kervella19}$^{18}$; \citet{peacock19}$^{19}$; \citet{endl08}$^{20}$;
\citet{muirhead18}$^{21}$; \citet{cutispoto02}$^{22}$; \citet{bochanski18}$^{23}$; \citet{nielsen19}$^{24}$;
\citet{bakos10}$^{25}$; \citet{bouchy05}$^{26}$; \citet{anglada12}$^{27}$; \citet{anglada13}$^{28}$;
\citet{delfosse13}$^{29}$; \citet{schoefer19}$^{30}$; \citet{butler06}$^{31}$; \citet{feng15}$^{32}$;
\citet{borosaikia16}$^{33}$; \citet{kervella08}$^{34}$; \citet{santos02}$^{35}$; \citet{vonbraun14}$^{36}$;
\citet{youngblood17}$^{37}$; \citet{boisse12}$^{38}$; \citet{pepe11}$^{39}$; \citet{bonfils05}$^{40}$;
\citet{vonbraun11}$^{41}$; \citet{cenarro07}$^{42}$; \citet{rosen16}$^{43}$; \citet{kochukhov20}$^{44}$;
\citet{gaspar16}$^{45}$; \citet{butler01}$^{46}$; \citet{santos04}$^{47}$; \citet{robertson12}$^{48}$
}
\end{deluxetable*}



 

